Deep Decarbonization of Multi-Energy Systems: A Carbon-Oriented Framework with Cross Disciplinary Technologies

The retirement of unabated coal power plants, the plummeting cost of renewable energy technologies, along with more aggressive public policies and regulatory reforms, are occurring at an unprecedented speed to decarbonize the power and energy systems towards the 2030 and 2050 climate goals. This article aims to establish a carbon-oriented framework to examine the role carbon emission is playing within a power grid that is rapidly transitioning to an integrated multi-energy system. We divide the carbon flows in the multi-energy systems into three stages: carbon allowances initialization/allocation, exchanging/pricing, and circulation. Then, we discuss how cross-disciplinary technologies, such as game theory, optimization, and machine learning can facilitate the modeling and analysis of the proposed framework.

==> Chenye.tex <==
Uncertainty is the primary reason for developing new methods to enable effective carbon allowance allocation, exchange, and circulation methods. The most straightforward way to manage uncertainties is to first conduct value prediction for all the uncertainty sources (e.g., demand prediction, price prediction, and renewable generation output prediction) and then decide based on the predicted values, e.g., in the optimization problems for energy producers and market operators as outlined in Section \ref{sec:carbon_allowance_exchange}. 

However, operations based on value predictions often lead to sub-optimal decision making, which warrants the distributional prediction enabled decision making, such as chance-constrained optimization, robust optimization, and more recently, the distributionally robust optimization \cite{9540759}. While such methods have been widely applied to the classical electric power system operation, e.g., economic dispatch and system planning, a multi-energy system contains more inter-dependent uncertainty sources. More uncertainty resources imply more flexibility in containing the carbon emission, while the uncertainty characterization (e.g., the chance constraints and the uncertainty sets) becomes much more challenging due to the inter-dependency.

One potential solution is to use advanced approximation toolboxes to decouple the inter-dependency utilizing the diverse temporal characteristics, yielding the multi-time scale system operation where the uncertainties in the power system are handled at the smaller time scale while the uncertainties in other energy systems (e.g., natural gas and heat) are managed at the larger time scale. An alternative to characterize the inter-dependent uncertainty is to utilize a data-driven approach. The CIF system with abundant data can well recover the true uncertainty set, guaranteed by the theoretical results from distributionally robust optimization based on the Wasserstein distance \cite{esfahani2018data}.
